Transductive Zero-Shot Learning using Cross-Modal CycleGAN

In Computer Vision, Zero-Shot Learning (ZSL) aims at classifying unseen classes -- classes for which no matching training image exists. Most of ZSL works learn a cross-modal mapping between images and class labels for seen classes. However, the data distribution of seen and unseen classes might differ, causing a domain shift problem. Following this observation, transductive ZSL (T-ZSL) assumes that unseen classes and their associated images are known during training, but not their correspondence. As current T-ZSL approaches do not scale efficiently when the number of seen classes is high, we tackle this problem with a new model for T-ZSL based upon CycleGAN. Our model jointly (i) projects images on their seen class labels with a supervised objective and (ii) aligns unseen class labels and visual exemplars with adversarial and cycle-consistency objectives. We show the efficiency of our Cross-Modal CycleGAN model (CM-GAN) on the ImageNet T-ZSL task where we obtain state-of-the-art results. We further validate CM-GAN on a language grounding task, and on a new task that we propose: zero-shot sentence-to-image matching on MS COCO.

==> finegrained.tex <==
\begin{table}[t]                                                                   
    \centering 
        \begin{tabular}{c | r r r r r r}
            Model & $\text{M}_{500}$& $\text{M}_{1000}$ & $\text{M}_{5000}$ & $\text{L}_{500}$ &$\text{L}_{1000}$ &$\text{L}_{5000}$ \\
            & & &  \\
    \hline
    CONSE %\cite{DBLP:journals/corr/NorouziMBSSFCD13}
    & 12.33 & 8.31 & 3.22 & 3.53 & 2.69 & 1.05 \\
    SYNC %\cite{DBLP:conf/cvpr/ChangpinyoCGS16}
    & \textbf{15.83} & 10.75 & 3.42 & \textbf{5.83} & 3.52 & 1.26\\ 
     Us & 15.74 & \textbf{11.03} & \textbf{3.95} & 5.19 & \textbf{3.8} & \textbf{1.51}\\
     \hline 
    \end{tabular} 
    \caption{ZSL task on fine-grained \textit{ImageNet-Full}. Measure: $F_{1}$}
    \label{finegrained}
\end{table}


==> mscoco2.tex <==
\begin{table}[t]                                   
    \centering 
        \begin{tabular}{c | c | c c c c}
           & Model & MFR & $F_{1}$ &$F_{5}$ & $F_{10}$ \\
    \hline 
    \multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Image To Text}}}& Random & 50 & 0.1 & 0.5& 1\\ 
    &Id & 20.3  & 3.3 & 13.9 & 23.5\\ 
    &CycleGan ($\lambda_c = 0)$& 21 & 4.2 & 15.7 & 25.2  \\
    &CycleGan ($\lambda_c = 1)$& \textbf{15.7} & \textbf{5.7} & \textbf{17.2} & \textbf{27.7}\\ 
    &CycleGan ($\lambda_c = 10)$ & 16.2 & 5 & 16.8& 26.6 \\ 
    &CycleGan ($\lambda_c = 100)$& 17.8 & 5.2 & 15.7 & 26 \\ 
    &CycleGan ($\lambda_c = 1000)$ &17.3 & 5.1 & 15.4 & 24.8\\ 
    &CycleGan ($\lambda_c = + \infty )$& 18.3 & 4.7 & 14.3& 24 \\
    &Supervised  &  \textit{7.3} & \textit{8.3} & \textit{26.3} & \textit{39.84}\\
     \hline 
     \hline 
   \multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Text to Image}}} &Random & 50 & 0.1 & 0.5& 1\\ 
    &Id & 14.1 & 2.8& 12.3 & 20.2 \\ 
    &CycleGan ($\lambda_c = 0)$& 14.1 & 3.1 & 15.1 & 23.7 \\
    &CycleGan ($\lambda_c = 1)$ & \textbf{11.1}& \textbf{4.1} & 15.5 & \textbf{27.7}\\
    &CycleGan ($\lambda_c = 10)$ &12.2 &3.6 & 15.5 & 26\\ 
    &CycleGan ($\lambda_c = 100)$ & 13.1 &2.9 & 12 & 21.7 \\ 
    &CycleGan ($\lambda_c = 1000)$ & 12 & 3.4 & 15.7 & 26.2\\ 
    &CycleGan ($\lambda_c = + \infty )$& 11.3 & 3.7 & \textbf{16.6} & 27.3 \\
    &Supervised & \textit{4.5} & \textit{7.1} & \textit{28.1} & \textit{44.7}\\
    \end{tabular} 
    \caption{Cross-modal results on MS COCO.}
    \label{mscoco}
\end{table}


==> sup_vs_unsup_g.tex <==
\begin{table*}[t]                                               \centering 
        \begin{tabular}{c | r r r r r r r r r }
            Model & $\text{M}_{500}$& $\text{M}_{1000}$ & $\text{M}_{5000}$ & $\text{L}_{500}$ &$\text{L}_{1000}$ &$\text{L}_{5000}$& $2_{hop}$ & $3_{hop}$ & All \\
            & & &  \\
    \hline
    Init. &  14.4& 15.3& 15.94 & 24.8 & 25.5 & 23.74 & 8.88 &12.37 & 15.35 \\
    cycle & \\ %comp/ucmr__dataset_ImageNet__multi_m0__lambda_cycle_gan_1__max_steps_2400/8qm2v46hs6
    c-gan &11.68 & 12.36 &13.06 &21.75 &22.05 & 20.86 & 7.34&10.73 &  13.34 \\
    gan   &12.05 & 12.68& 13.42 & 22.72& 23.52&22.44 & 7.51& 11.41& 14.25\\
    sup&  9.4 & 9.8 & 10.46 &19.2 & 20 & 17.88 & 5.83& 8.88  & 11.07 \\
    sup + sup & \\  %comp/ucmr__dataset_ImageNet__multi_m1__lambda_supervised_1__max_steps_10000/iab479gnxp
    Fin ($\lambda_c=0$) & \\ %comp/ucmr__dataset_ImageNet__multi_m3__identity_True__max_steps_0__nb_layer_1/n9hy695bgx
    Fin &  \textbf{8.2} &  \textbf{8.4} &  \textbf{9.06}&  \textbf{17.4} &  \textbf{18.1} &  \textbf{16.14} &  \textbf{5.17} &  \textbf{8.23} &  \textbf{9.98}\\ 
    \hline 
    \hline
    Init. & 13.6 & 15.2 & 16.1 & 31.2 & 31.2 & 26.02 & 9.88 & 12.71 & 15.65 \\
    cycle & \\ %comp/ucmr__dataset_ImageNet__multi_m0__lambda_cycle_gan_1__max_steps_2400/g9nz5505a0 
    c-gan & 10.66&11.78 &12.8 & 23.94 & 24.02&21.52  &7.72 &10.79 &  13.32 \\
    gan  &  10.8& 11.81 & 12.82&23.83  & 24.47& 22.23 &7.57 & 11.03&  13.68 \\
    sup&  8.4 & 8.45 & 10.35 & 20.33 & 21.2 & 18.4 & 6.06 & 8.87 & 11.13 \\
    sup + sup & \\ %comp/ucmr__dataset_ImageNet__multi_m1__lambda_supervised_1__max_steps_10000/6tqml0r24t
    Fin ($\lambda_c=0$) & \\ %comp/ucmr__dataset_ImageNet__multi_m3__identity_True__max_steps_0__nb_layer_1/qu1s62h84r
    Fin  & \textbf{7.4} & \textbf{7.95} & \textbf{8.93} & \textbf{17.4} & \textbf{18.1} & \textbf{16.1} & \textbf{5.3} & \textbf{8.17} & \textbf{9.97} \\
    \end{tabular} 
    \caption{Ablation study. Up: Zero-shot Learning. Down: Generalized ZSL. Measure: MFR.}
    \label{sup_vs_unsup}
\end{table*}



==> word_500.tex <==
\begin{table}[t]                                                                   
    \centering 
        \begin{tabular}{c | c c c c c c }
            Model & MEN & SemSim & SimLex & VisSim & WordSim & USF\\
    \hline
    $X$ & 72 & 68 & 29 & 54 & 61 & 21\\ 
    $\text{sup}_1(X)$ & \textbf{73} & 68 & \textbf{32} & \textbf{58} & 61 & 21 \\
    
    $\text{cgan}_2(X)$ & 72 & 70 & 27 & 56 & 61 & 20  \\
    $\text{sup}_3 \circ \text{cgan}_2(X)$ & \textbf{73} & 68 & 31 & \textbf{58} & 62 & 21\\
    $\text{cgan}_4 \circ \text{cgan}_2(X)$ & \textbf{73} & \textbf{72} & 27 & \textbf{58} & \textbf{63} & 21\\
    $\text{sup}_5 \circ \text{cgan}_4 \circ \text{cgan}_2(X)$ & 72 & 67 & 31 & 57 & 59 & \textbf{22}\\
    $\text{cgan}_6 \circ \text{cgan}_4 \circ \text{cgan}_2(X)$ & 72 & 70 & 27 & 57 & \textbf{63} & \textbf{22}\\
    \hline 
    \end{tabular} 
    \caption{Evaluation grounded word representations ($d=500$)}
    \label{word_500}
\end{table}


==> word_500_2.tex <==
\begin{table}[t]                                                                   
    \centering 
        \begin{tabular}{c | c c c c c c c |c}
            Model & MEN & SemSim & SimLex & VisSim & WordSim & USF & Conc. & Avg. \\
    \hline
    $X$ & 72 & 68 & 29 & 54 & 61 & 21\\ 
    $T_1(X)$ & \textbf{73} & 68 & \textbf{32} & \textbf{58} & 61 & 21 \\
    
    $\hat{V}_2(X)$ & 72 & 70 & 27 & 56 & 61 & 20  \\
    $T_3 \circ \hat{V}_2(X)$ & \textbf{73} & 68 & 31 & \textbf{58} & 62 & 21\\
    $\hat{V}_4(X)$ & \textbf{73} & \textbf{72} & 27 & \textbf{58} & \textbf{63} & 21\\
    $T_5 \circ \hat{V}_4(X)$ & 72 & 67 & 31 & 57 & 59 & \textbf{22}\\
    $\hat{V}_6(X)$ & 72 & 70 & 27 & 57 & \textbf{63} & \textbf{22}\\
    \hline 
    \end{tabular} 
    \caption{Evaluation of grounded word representations ($d=500$)}
    \label{word_500}
\end{table}

